Koopman pose predictions for temporally consistent human walking estimations

We tackle the problem of tracking the human lower body as an initial step toward an automatic motion assessment system for clinical mobility evaluation, using a multimodal system that combines Inertial Measurement Unit (IMU) data, RGB images, and point cloud depth measurements. This system applies the factor graph representation to an optimization problem that provides 3-D skeleton joint estimations. In this paper, we focus on improving the temporal consistency of the estimated human trajectories to greatly extend the range of operability of the depth sensor. More specifically, we introduce a new factor graph factor based on Koopman theory that embeds the nonlinear dynamics of several lower-limb movement activities. This factor performs a two-step process: first, a custom activity recognition module based on spatial temporal graph convolutional networks recognizes the walking activity; then, a Koopman pose prediction of the subsequent skeleton is used as an a priori estimation to drive the optimization problem toward more consistent results. We tested the performance of this module on datasets composed of multiple clinical lowerlimb mobility tests, and we show that our approach reduces outliers on the skeleton form by almost 1 m, while preserving natural walking trajectories at depths up to more than 10 m.

==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}


==> preamble/courseFormatting.tex <==
%make underscore work without escaping in text mode
\usepackage{underscore}

%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue3}\sffamily}

%Perfect 1-inch margins
\usepackage[margin=1in]{geometry}
\usepackage[medium,compact]{titlesec}
\usepackage{longtable}
\titleformat*{\section}{\titlestyle \Large}
\titleformat*{\subsection}{\titlestyle \large \itshape}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}

%Displayed quotations (used to define an environment for function specification)
\usepackage{csquotes}


%Include code
\usepackage{listings}

%formatting for the description of a function's input/output arguments
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}

\newcommand{\dstar}{$\bigstar$}


==> preamble/courseProblemSet.tex <==
\input{preamble/courseFormatting}

%Facilities for markers file
% open file the beginning of the document
\AtBeginDocument{%
  \newwrite\markerstream
  \immediate\openout\markerstream=\jobname.mlg
}
% close the file at the end of the document
\AtEndDocument{%
  \immediate\closeout\markerstream
}
%definition similar to \typeout, but for markers
\makeatletter
\newcommand{\markerout}[1]{\begingroup \set@display@protect \immediate \write \markerstream {#1}\endgroup}
\makeatother

\usetikzlibrary{intersections}

\titleformat{\section}{\titlestyle\large\bfseries}{Problem \thesection:}{0.5ex}{}
%\titleformat{\subsection}{\normalfont\bfseries}{Problem \thesubsection:}{0.5ex}{}
\titleformat{\paragraph}[runin]{\titlestyle\normalsize\bfseries}{}{2pt}{}

%Macro for paragraph header for preparation steps to questions
%\newcommand{\preparation}{\smallskip\par\noindent\textbf{\titlestyle Preparation.~}}

\newcommand{\preparation}[1][]{%
\smallskip\par\noindent%
\textbf{\titlestyle Preparation \displayifnotempty{~(}{#1}{)}.~}}

%New custom counter for question
\newcounter{question}[section]

%Macro for writing points for the current question to the log file.
\newcommand{\pointmarker}{\typeout{Question points marker [\thesection.\thequestion] [\questionpoints]}}

\makeatletter
%Makes questions that:
%- are automatically numbered using the format <sectionNumber>.<questionNumber>
%- can be referred to using the usual \label-\ref mechanism
%- if the optional argument is not empty, this is displayed in parenthesis (typically, this will be a \points{n} or a \optional command). If the optional argument is empty, a single point is silently added to the point counter.
\newcommand{\question}[1][]{%
\smallskip\par\noindent%
\refstepcounter{question}\zerovar{\questionpoints}%
\sbox\boxifnotempty{\textbf{\titlestyle #1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
\textbf{\titlestyle Question \thesection.\thequestion\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
\ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
\def\@currentlabel{{\thesection.\thequestion}}\pointmarker}
\makeatother
\newcommand{\hintquestion}[1]{\paragraph{Hint
    for question \ref{#1}:~}}
\newcommand{\hint}{\paragraph{Hint:~}}

\newcommand{\answer}[1][]{\smallskip\leavevmode\\\noindent\textbf{Answer \thesection.\thequestion#1:~}}

\newcommand{\updated}[1]{{\color{red} #1}}

\newcolorlabel{labeloptional}{DodgerBlue3}
\newcommand{\optional}{\labeloptional{optional}}
\newcolorlabel{labelprovided}{Orange1}
\newcommand{\provided}{\labelprovided{provided}}
\newcolorlabel{labelvideo}{OliveDrab3}
\newcommand{\video}{\labelvideo{video}}
\newcolorlabel{labelimage}{DarkOrchid2}
\newcommand{\image}{\labelimage{image}}
\newcolorlabel{labelcode}{SlateBlue2}
\newcommand{\code}{\labelcode{code}}
\newcolorlabel{labelscan}{Chocolate3}
\newcommand{\scan}{\labelcode{scan}}
\newcolorlabel{labelnew}{OliveDrab3}
\newcommand{\lbnew}{\labelnew{new}}

%\newcommand{\optional}{{\titlestyle optional}}

\tikzset{point/.style={inner sep=0pt,fill=black,circle,minimum size=4pt}}

%macros for keeping track of points (total, and for current question)
\zerovar{\totalpoints}
\zerovar{\bonuspoints}
\zerovar{\questionpoints}
\newcommand{\increasepoints}[1]{\addtovar{\totalpoints}{#1}\addtovar{\questionpoints}{#1}}
\newcommand{\points}[1]{#1 point\ifthenelse{\equal{#1}{1}}{}{s}\increasepoints{#1}}
\makeatletter
\newcommand{\totalpointswithbonus}[1]{\pgfmathparse{\storeddef{totalpoints}+#1}\pgfmathresult\typeout{Total points marker [\pgfmathresult]}}
\makeatother

\newstoreddef{totalpoints} %remember total number of points in aux file

% answer boxes
\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\par\bigskip{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}

% text fields
\newcommand{\textrowfield}[1]{\par\noindent#1: \enspace\hrulefill}

% formatting for the description of a function's input/output arguments
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
\mdfdefinestyle{classspecification}{%
linecolor=DarkOliveGreen3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
%Note: I was not able to avoid duplication of options.

\newenvironment{functionspecification}{\markerout{Marker function [start]}\begin{mdframed}[style=functionspecification]}
{\markerout{Marker function [end]}\end{mdframed}}%
\newenvironment{classspecification}{\markerout{Marker class [start]}\begin{mdframed}[style=classspecification]}
{\markerout{Marker class [end]}\end{mdframed}}%
%\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\newenvironment{cdescription}{\fdescription}{\endfdescription}
\NewEnviron{frequirements}{\par\noindent{\titlestyle Requirements}: \BODY\markerout{Marker text [requirements] [start]^^J\BODY^^JMarker text [requirements] [end]}\par}
\newcommand{\cname}[1]{\noindent{\titlestyle Class name}: \var{#1}\par}
\newenvironment{finputs}{\markerout{Marker argument_group [start] [inputs]}\noindent{\titlestyle Input arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foutputs}[1][Output]{\markerout{Marker argument_group [start] [outputs]}\noindent{\titlestyle #1 arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newcommand{\freturns}[2][]{\noindent{\titlestyle Returns}: \var{#2}\displayifnotempty{ (type }{\var{#1}}{)}}
\newcommand{\argument}[4][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2} %
  \ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [#4]}dim. \vardim{#3}{#4}\ifnotempty{#1}{, }}%
  \displayifnotempty{\markerout{Marker argument [type] [#1]}type }{\var{#1}}{})}\markerout{Marker argument [end]}}
\newcommand{\argumentscalar}[2][]{\argument[#1]{#2}{}{}}
\newcommand{\fheader}[3][]{\noindent{\titlestyle Header}: \function[#1]{#2}{#3}\par}
\newcommand{\fname}[2][Function]{\noindent{\titlestyle #1 name}: \var{#2}\par}
\newcommand{\ffilename}[1]{\noindent{\titlestyle File name}: \file{#1}\par}
\newcommand{\functionheader}[3][]{\markerout{Marker function_header [#1] [#2] [#3]}\function[#1]{#2}{#3}\par}

%ROS node specification
\newenvironment{nodespecification}{\begin{mdframed}[style=functionspecification]%
\newcommand{\filename}[1]{\par{\titlestyle File name:} \file{##1}}
\renewenvironment{description}{\par\noindent{\titlestyle Description:}}{\par}%
\newenvironment{subscribers}{\par\noindent{\titlestyle Subscribes to topics:}}{}%
\newenvironment{publishers}{\par\noindent{\titlestyle Publishes to topics:}}{}%
%
}{\end{mdframed}}

\newcommand{\rostopic}[2]{\var{#1} (type \var{#2})}

% Macros for questions where student need to draw on axes
\newcommand{\drawingaxes}[1][]{\draw[gray] (-5,-5) grid (5,5);
  \draw[very thick, -latex] (-5.7,0) -- (5.7,0);
  \draw[very thick, -latex] (0,-5.7) -- (0,5.7); #1}
\newcommand{\shifteddrawingaxes}[1][]{
  \begin{scope}[xshift=15cm]
    \drawingaxes[#1]
  \end{scope}
}

\newcommand{\drawexercise}[2][]{\begin{center}
\begin{tikzpicture}[scale=0.6]
  \node[text width=5cm,anchor=west]{#2};
  \shifteddrawingaxes[#1]
\end{tikzpicture}
\end{center}
}


==> preamble/courseProblemSetSectionsLettered.tex <==
%Change format of numbering for questions to letters instead of numbering
\renewcommand{\thequestion}{\alph{question}}


==> preamble/courseSyllabus.tex <==
 \input{preamble/courseFormatting}


\newlength{\topicwidth}
\newlength{\topicdatewidth}
\setlength{\topicdatewidth}{19mm}
\newlength{\duewidth}
\setlength{\duewidth}{23mm}

%Create a topictable environment from the longtable environment
\newenvironment{topictable}[1][2cm]%
{\newcommand{\picswidth}{#1}\setlength{\topicwidth}{\textwidth-\picswidth-\topicdatewidth-\duewidth-12.5mm}%
\setcounter{topic}{1}\begin{longtable}{p{\picswidth}p{\topicwidth}p{\topicdatewidth}p{\duewidth}}}%
{\end{longtable}}

%Prepare counter and relative macros for handling array of class dates
\newcount\i
\pgfmathsetcount{\i}{0}
\def\classdate{\pgfprint{\classdatearray[\i]}\global\advance\i 1\relax}

%Counters for topic and subtopic
\newcounter{topic}
\newcounter{subtopic}

%Topichead
\def\topichead#1#2#3{\rowcolor{SlateGray1}{\setcounter{subtopic}{1}\rule{0pt}{16pt}\titlestyle Topic \arabic{topic}\addtocounter{topic}{1}} & \multicolumn{3}{l}{{\titlestyle #1:} #2 \rule[-8pt]{0pt}{12pt}}\\\tikz[overlay]{\node[anchor=north west,inner sep=0pt]{\includegraphics[width=\picswidth,keepaspectratio]{figures/#3}};}}
\def\firstsubtopic#1{ & \makecell[{{p{\topicwidth}}}]{\rule{0pt}{14pt}#1}\addtocounter{subtopic}{1}}
\def\subtopic#1{\\ \cmidrule{2-4} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
%\def\topicdate#1{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\newcommand{\topicdate}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\def\due#1{& \makecell[{{p{\duewidth}}}]{#1}}
\def\endtopic{\\}
\newcolorlabel{labelhw}{Orange1}
\newcommand{\hwdue}[1]{\labelhw{HW #1}}
\newcolorlabel{paperdue}{Tomato1}
\newcolorlabel{examdue}{Tomato1}
\newcolorlabel{labelMH}{DodgerBlue3}
\newcommand{\mhday}{\labelMH{M-H}~}
\newcolorlabel{labelqz}{Sienna3}
\newcommand{\qzdue}[1]{\labelqz{QZ #1}~}

%TODO: Add automatic test to check if a subtopic is the first subtopic, and adjust the formatting accordingly.
%The subtopic counter is already there, but due to conflicts with the tabular environment, I was not able to include the test inside the \subtopic macro.
%\def\tpctest{\noalign{\ifnum\value{subtopic}=1{}\else{\hrule}\fi}}


==> preamble/generateGraphLocalization <==
#!/usr/bin/env python
# Note: in the list of node and edge quantities: first element is the name to use in the command name,
# the second is the one to use in the definition

import os
f=open('graphLocalization.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Notation for nodes\n')
nodeIndexList=['i','j']
nodeStateDoubleList=[['R','R'],['T','T']]
for index in nodeIndexList:
    for state in nodeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
        f.write('\\newcommand{\\d'+state[0]+index+'}{\\dot{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dd'+state[0]+index+'}{\\ddot{'+state[1]+'}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

edgeIndexList=['ij','ji']
edgeStateDoubleList=[['R','R'],['T','T'],['beta','\\beta'],['c','c'],['d','d'],['q','q'],['l','\\lambda'],['varphi','\\varphi'],['g','g']]

f.write('% Notation for edges\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Notation for edges, measured quantities\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\t'+state[0]+index+'}{\\tilde{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dt'+state[0]+index+'}{\\dot{\\tilde{'+state[1]+'}}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Node state differences\n')
f.write('\\newcommand{\\xjmi}{x_j-x_i}\n')
f.write('\\newcommand{\\vjmi}{v_j-v_i}\n')
f.write('\\newcommand{\\nxjmi}{\\norm{\\xjmi}}\n')
f.write('\n')

f.write('% Notation for desired quantities\n')
quantityTripleList=[['x','x','i'],['x','x','j'],['beta','\\beta','ij'],['d','d','ij']]
for quantity in quantityTripleList:
    f.write('\\newcommand{\\'+quantity[0]+'g'+quantity[2]+'}{'+quantity[1]+'_{g,'+quantity[2]+'}}\n')

f.close()






        


==> preamble/generateNotation <==
#!/usr/bin/env python
import string
import os
f=open('notation.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Shortand notation for vectors and their derivatives\n')
for c in string.ascii_lowercase+string.ascii_uppercase:
    f.write('\\providecommand{\\v'+c+'}{\\vct{'+c+'}}\n')
    f.write('\\providecommand{\\dv'+c+'}{\\dot{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\tv'+c+'}{\\tilde{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\dtv'+c+'}{\\dot{\\tilde{\\vct{'+c+'}}}}\n')
f.write('\n')
for c in [['beta','\\beta'],['sigma','\\sigma']]:
    f.write('\\providecommand{\\v'+c[0]+'}{\\boldsymbol{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dv'+c[0]+'}{\\dot{\\boldsymbol{'+c[1]+'}}}\n')
f.write('\n')
for c in ['e']:
    f.write('\\providecommand{\\t'+c+'}{\\tilde{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for derivatives and bold of symbols\n')
for c in [['gamma','\\gamma'],['Delta','\Delta']]:
    f.write('\\providecommand{\\d'+c[0]+'}{\\dot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dd'+c[0]+'}{\\ddot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\v'+c[0]+'}{\\bm{'+c[1]+'}}\n')
f.write('\n')


f.write('% Shortand notation for matrices\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\m'+c+'}{\\vct{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for calligraphic upper case letters\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\c'+c+'}{\\mathcal{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for some tilded symbols and their derivatives\n')
symbolDoubleList=[['x','x'],['y','y'],['varphi','\\varphi']]
for symbol in symbolDoubleList:
    f.write('\\providecommand{\\t'+symbol[0]+'}{\\tilde{'+symbol[1]+'}}\n')
    f.write('\\providecommand{\\dt'+symbol[0]+'}{\\dot{\\tilde{'+symbol[1]+'}}}\n')
f.write('\n')

f.close()


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
  \begin{tikzpicture}[scale=0.7]%
    \input{sketch/#1}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
\input{tikz/#1}%
\endpgfgraphicnamed%
}


==> preamble/math.tex <==
%AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage[cmex10]{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother

\usepackage{mathtools}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

==> preamble/reviewDraft.tex <==
\usepackage{background}
\backgroundsetup{contents={%
    \begin{tikzpicture}[overlay,font=\sffamily]
      \newcommand{\scaletop}{-.68in}
      \newcommand{\scalepitch}{1.15em}
      \newcommand{\scaleoffset}{.5in}
      \foreach \x in {1,...,60}{
        \node at ($(current page.north west)+(\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+\x)}\pgfmathresult};
        \node at ($(current page.north east)+(-\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+100+\x)}\pgfmathresult};
      }
      \node at ($(current page.south)+(0,.5in)$) {*** For Review Only ***};
    \end{tikzpicture}
  },color=blue,scale=1,angle=0}

\author{\textcolor{blue}{\sffamily Author Names Omitted for Anonymous Review}}
\renewcommand{\author}[1]{}


==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}

